On Deleting Vertices to Reduce Density in Graphs and Supermodular Functions

We consider deletion problems in graphs and supermodular functions where the goal is to reduce density. In Graph Density Deletion (GraphDD), we are given a graph $G=(V,E)$ with non-negative vertex costs and a non-negative parameter $\rho \ge 0$ and the goal is to remove a minimum cost subset $S$ of vertices such that the densest subgraph in $G-S$ has density at most $\rho$. This problem has an underlying matroidal structure and generalizes several classical problems such as vertex cover, feedback vertex set, and pseudoforest deletion set for appropriately chosen $\rho \le 1$ and all of these classical problems admit a $2$-approximation. In sharp contrast, we prove that for every fixed integer $\rho > 1$, GraphDD is hard to approximate to within a logarithmic factor via a reduction from Set Cover, thus showing a phase transition phenomenon. Next, we investigate a generalization of GraphDD to monotone supermodular functions, termed Supermodular Density Deletion (SupmodDD). In SupmodDD, we are given a monotone supermodular function $f:2^V \rightarrow \mathbb{Z}_{\ge 0}$ via an evaluation oracle with element costs and a non-negative integer $\rho \ge 0$ and the goal is remove a minimum cost subset $S \subseteq V$ such that the densest subset according to $f$ in $V-S$ has density at most $\rho$. We show that SupmodDD is approximation equivalent to the well-known Submodular Cover problem; this implies a tight logarithmic approximation and hardness for SupmodDD; it also implies a logarithmic approximation for GraphDD, thus matching our inapproximability bound. Motivated by these hardness results, we design bicriteria approximation algorithms for both GraphDD and SupmodDD.

==> intro-sections/intro-deprecated.tex <==
\section{Introduction}\label{sec:introduction}
\label{sec:intro}
The \emph{densest subgraph} problem in graphs (\dsg) is a core primitive in graph and network mining applications. In \dsg, we are given a graph $G=(V,E)$ and the goal is to find $\lambda_G^*:=\max_{S\subseteq V}|E(S)|/|S|$, where $E(S)$ is the set of edges with both end vertices in $S$. 
\dsg is not only interesting for its applications but is a fundamental problem in algorithms and combinatorial optimization with several connections to graph theory, matroids, and submodularity. Many recent works have explored various aspects of \dsg and related problems from both theoretical and practical perspectives \cite{densest-subgraph-survey,boob-20,sw-20,vbk-21,cqt-22,hqc-22,dhulipala2022differential,dinitz2023improved,adaptive-orientations,ne-24}. A useful feature of \dsg is its polynomial-time solvability. This was first seen via a reduction to network flow \cite{g-84,Picard-Queyranne} but another way to see it is by considering a more general problem, namely the \emph{densest supermodular subset} problem (\dss): Given a supermodular function $f:2^V\rightarrow \R_{\ge 0}$ via evaluation oracle, the goal is to find $\lambda^*_f:=\max_{S \subseteq V} {f(S)}/{|S|}$.
One can easily see that \dsg is a special case of \dss by noting that for any graph $G$, the function $f:2^V \rightarrow \mathbb{Z}$ defined by $f(S) = |E(S)|$ for every $S\subseteq V$ is a supermodular function. It is well-known and easy to see that \dss and \dsg can be solved in polynomial-time by a simple reduction to submodular function minimization. Several other problems that are studied in graph and network mining can be seen as special cases of \dss. Recent work has demonstrated the utility of the supermodularity lens in understanding greedy heuristics and approximation algorithms for \dsg and these problems \cite{cqt-22,vbk-21,hqc-22,hqc-23}.

\paragraph{Density Deletion Problems.} In this work we consider several interrelated \emph{vertex deletion} problems that aim to \emph{reduce} the density. 
We start with the graph density deletion problem. %For a fixed constant $\rho$, we consider \rhodds{\rho} as defined below. 
\begin{definition}[\rhodds{\rho}] For a fixed constant $\rho$, the $\rho$-graph density deletion problem, denoted \rhodds{\rho}, is defined as follows:
    \begin{mdframed}
\begin{tabular}{ l l }
 \emph{\textbf{Input}:} &  Graph $G=(V, E)$ and vertex costs $c:V\rightarrow\R_{\ge 0}$ \vspace{1mm}\\  
 \emph{\textbf{Goal}:} & $\arg \min\{\sum_{u\in S}c_S : S\subseteq V \text{ and } \lambda^*_{G-S} \le \rho\}$. 
\end{tabular}
\end{mdframed}
\end{definition}
This deletion problem naturally generalizes to supermodular functions as defined below. We recall that a set function $f: 2^V\rightarrow \R$ is (i) submodular if $f(A)+f(B)\ge f(A\cap B) + f(A\cup B)$ for every $A, B\subseteq V$, (ii) supermodular if $-f$ is submodular, (iii) non-decreasing if $f(A)\le f(B)$ for every $A\subseteq B\subseteq V$, and (iv) normalized if $f(\emptyset)=0$. We observe that non-negative normalized supermodular functions are non-decreasing. For a function $f: 2^V\rightarrow R$ and $S\subseteq V$, we define $f_{V-S}$ as the function $f$ restricted to the ground set $V-S$. The evaluation oracle for the function takes a subset $S\subseteq V$ as input and returns the function value of the set $S$. %For a fixed constant $\rho$, we define \rhosdds{\rho} below. 
\begin{definition}[\rhosdds{\rho}] For a fixed constant $\rho$, the $\rho$-supermodular density deletion problem, denoted \rhosdds{\rho}, is defined as follows:
    \begin{mdframed}
\begin{tabular}{ l l }
 \emph{\textbf{Input}:} &  Integer-valued normalized supermodular function $f:2^V\rightarrow\Z_{\ge 0}$ via evaluation oracle and \\
 & element costs $c:V\rightarrow\R_{\ge 0}$ \vspace{1mm}\\  
  % & \\
 \emph{\textbf{Goal}:} & $\arg \min\{\sum_{u\in S}c_u : S\subseteq V \text{ and } \lambda^*_{f_{V-S}} \le \rho\}$. 
\end{tabular}
\end{mdframed}
\end{definition}
When the density threshold $\rho$ is part of input, we use \dds and \sdds to refer to these problems. It is easy to see that \dds (and hence \sdds) is NP-Hard from a general result on vertex deletion problems \cite{Lewis_Yannakakis_1980}. Our goal is to understand the approximability of these problems.

\paragraph{Motivations and Connections.}
While the deletion problems are natural in their formulation, to the best of our knowledge, \dds has only recently been explicitly defined and explored. Bazgan, Nichterlein and Vazquez Alferez \cite{bazgan_et_alSWAT2024} defined and studied this problem from an FPT perspective.  As pointed out in their work, given the importance of DSG and DSS in various applications to detect communities and sub-groups of interest, it is useful to consider the robustness (or sensitivity) of the densest subgraph to the removal of vertices. In this context, we mention the classical work of Cunningham on the attack problem \cite{Cunningham85} which
can be seen as the problem of deleting \emph{edges} to reduce density;
this edge deletion problem can be solved in polynomial time for integer parameters $\rho$ via matroidal and network flow techniques. In addition to their naturalness and the recent work, we are motivated to consider \dds and \sdds owing to their connections to several classical vertex deletion problems as well as a matroidal structure underlying \dds that we articulate next.

We observe that \rhodds{0} is equivalent to the vertex cover problem: requiring density of $0$ after deleting $S$ is equivalent to $S$ being a vertex cover of $G$.  One can also see, in a similar fashion, that \rhodds{1} is equivalent to the pseudoforest deletion set problem, denoted \pfds---where the goal is to delete vertices so that every connected component in the remaining graph has at most one cycle, and \rhodds{(1 - 1/|V|)} is equivalent to the feedback vertex set problem, denoted \fvs---where the goal is to delete vertices so that the remaining graph is acyclic. Vertex cover, \PFDS, and \FVS admit $2$-approximations, and moreover this bound cannot be improved under the Unique Games Conjecture (UGC) \cite{KhotR08}. We note that while $2$-approximations for vertex cover is relatively easy, $2$-approximations for \fvs and \pfds are non-obvious \cite{Bafna-Berman-Fujito95,BG96,CHUDAK1998111}. 
Until very recently there was no polynomial-time solvable linear program (LP) that yielded a $2$-approximation for \fvs and \pfds.  
In fact, the new and recent LP formulations \cite{chandrasekaran2024polyhedralaspectsfeedbackvertex} for \fvs and \pfds are obtained via the connection to Charikar's LP-relaxation for \dsg \cite{charikar_greedy_2000}.  Fujito \cite{Fujito-matroid-fvs} unified the $2$-approximations for vertex cover, \fvs, and \pfds via primal-dual algorithms %for vertex cover, \fvs, and \pfds 
by considering a more general class of \emph{matroidal} vertex deletion problem on graphs that is relevant to our work. This abstract problem, denoted \mfvs\footnote{We use the 
\emph{feedback vertex set} terminology in our naming of the \mfvs problem since the goal is to pick a min-cost subset of vertices to cover all \emph{circuits} of the matroid defined on the edges of a graph. This generalizes \fvs which is \mfvs where the matroid of interest is the graphic matroid on the input graph.}, 
is defined below. 
\begin{definition}[\mfvs] The Matroid Feedback Vertex Set problem, denoted \mfvs, is defined as follows:
    \begin{mdframed}
\begin{tabular}{ l l }
 \emph{\textbf{Input}:} &  Graph $G=(V, E)$, vertex costs $c:V\rightarrow\R_{\ge 0}$, and  \\ 
 & Matroid $\calM = (E, \calI)$ with $\calI$ being the collection of independent sets \\
 & \quad \quad (via an independence testing oracle)
 \vspace{1mm}\\  
  % & \\
 \emph{\textbf{Goal}:} & $\arg \min\{\sum_{u\in S}c_u : S\subseteq V \text{ and } E[V-S] \in \calI\}$. 
\end{tabular}
\end{mdframed}
\end{definition}
Fujito \cite{Fujito-matroid-fvs} obtained a $2$-approximation for \mfvs for the class of ``uniformly sparse'' matroids \cite{Lee_Streinu_2008}. 
It is not difficult to show that vertex cover, \fvs, and \pfds can  be cast as special cases of \mfvs 
where the associated matroids are ``uniformly sparse''.  Consequently, Fujito's result unifies the $2$-approximations for these three fundamental problems. 

We now observe some non-trivial connections between $\rho$-\dds, \mfvs and \rhosdds{\rho}. We can show that $\rho$-\dds is a special case of \mfvs for every integer $\rho$: indeed, $\rho$-\dds corresponds to \mfvs where the matroid $\calM_\rho$ is the $\rho$-fold union of the $1$-cycle matroid defined on the edge set of the input graph (see \Cref{thm:dds-to-matroidfvs} in \Cref{appendix:sec:reductions}). Although it is not obvious, we can show that \mfvs is a special case of \rhosdds{1} (see \Cref{thm:matroidfvs-to-supmodDD} in \Cref{appendix:sec:reductions}). 
%a subset of edges is independent if and only if each component induced by the subset has at most one cycle
We refer the reader to the problems in the right column in Figure \ref{fig:reductions}(b) for a pictorial representation of the reductions discussed so far. 
Given these connections and the existence of a $2$-approximation for vertex cover, \fvs, and \pfds, we are led to the following questions. 

\begin{question}\label{question:main}
  What is the approximability of $\rho$-\dds, \mfvs, and $\rho$-\sdds? Do these admit a constant factor approximation?
\end{question}

\subsection{Results} 
In this section, we give an overview of our technical results that resolve Question~\ref{question:main} up to a constant factor gap.
\subsubsection{Connections between \submodcover and \sdds}
We obtain a logarithmic approximation for \rhodds{\rho}, \mfvs, and \rhosdds{\rho} via a reduction to the
submodular cover problem and using the Greedy algorithm for it due to Wolsey \cite{Wolsey82}. 
First, we recall the submodular cover problem. 
\begin{definition}[\submodcover] The submodular cover problem, denoted \submodcover, is defined as follows:
    \begin{mdframed}
\begin{tabular}{ l l }
 \emph{\textbf{Input}:} &  Integer-valued normalized non-decreasing submodular function $h:2^V\rightarrow\Z_{\ge 0}$ \\
 & via evaluation oracle and \\ 
    & element costs $c:V\rightarrow\R_{\ge 0}$ \vspace{1mm}\\  
 \emph{\textbf{Goal}:} & $\arg \min\{\sum_{e\in F}c_e : F \subseteq V \text{ and } h(F) \ge h(V)\}$. 
\end{tabular}
\end{mdframed}
\end{definition}

For a function $f: 2^V\rightarrow \R$, we define the marginal $f(v|S):=f(S+v) - f(S)$ for every $v\in V$ and $S\subseteq V$. 
We show the following result. 

\begin{restatable}{theorem}{thmsddsToSubmodCover}\label{thm:sddsToSubmodCover}
Let $f: 2^V\rightarrow \Z_{\ge 0}$ be an integer-valued normalized supermodular function and $\rho$ be a rational number. Then, there exists a normalized non-decreasing submodular function $h:2^V\rightarrow\R_{\geq 0}$ such that 
\begin{enumerate}
    \item if $\rho$ is an integer, then $h$ is integer-valued, 
    % \knote{added this. Edit the proof accordingly.}
    \item for $F\subseteq V$, we have that $\lambda^*_{f|_{V-F}} \leq \rho$ if and only if $h(F)\ge h(V)$, 
    \item $h(v) \leq \max\{0, f(v|V - v) - \rho\}$ for all $v \in V$, and 
    \item evaluation queries for the function $h$ can be answered in polynomial time by making polynomial number of  evaluation queries to the function $f$. 
\end{enumerate}
\end{restatable}


We discuss the consequences of Theorem \ref{thm:sddsToSubmodCover} for \rhosdds{\rho}. 
We recall that \submodcover admits a
% $O(\log{(\max_{v} h(v))})$-approximation 
$(1 + \ln{(\max_{v} h(v))})$-approximation 
for input function $h$ via the Greedy algorithm of Wolsey \cite{Wolsey82}. 
% \cnote{Wolsey's result is precise - $(1+ \ln \max_v h(v))$ - should we cite it that way?}. 
Consider \rhosdds{\rho} for integer-valued $\rho$. 
%By Theorem \ref{thm:sddsToSubmodCover} and the additional observation that the function $h$ defined in the theorem is integer-valued
By Theorem \ref{thm:sddsToSubmodCover}, we have a reduction to \submodcover and consequently, we have a 
% $O(\log(\max_{v\in V} f(v|V-v)))$-approximation. 
$(1 + \ln(\max_{v\in V} f(v|V-v)))$-approximation. 
In particular, we note that \rhodds{\rho} for integer-valued $\rho$ and \mfvs admit $O(\log{n})$-approximation, where $n$ is the number of vertices in the input graph. 
\iffalse
We mention that if $\rho$ is a rational value, say $\rho=p/q$, then we 
%Next, consider \rhosdds{\rho} for rational $\rho=p/q$. We 
may reduce it to an instance of \rhosdds{\rho} with integer-valued $\rho$ by scaling the input function by $q$; if $\rho$ is irrational, then \rhosdds{\rho} has additional complications and cannot be simply handled by scaling. 
\fi

\begin{corollary}\label{coro:rhodds-and-mfvs}
    \rhosdds{\rho} for integer-valued $\rho$ admits an 
    % $O(\log{(\max_{v\in V}f(v|V-v))})$-approximation.
    $(1 + \ln{(\max_{v\in V}f(v|V-v))})$-approximation, where $f:V\rightarrow\Z_{\ge 0}$ is an integer-valued normalized supermodular function.
    Consequently, \rhodds{\rho} for integer valued $\rho$ and \mfvs admit $O(\log{n})$-approximations, where $n$ is the number of vertices in the input graph. 
\end{corollary}

\begin{remark}
The reduction from \sdds to \submodcover is in some sense implicit in prior literature (see \cite{Ueno_Kajitani_Gotoh_1988, Fujito-matroid-fvs} for certain special cases of supermodular functions).
We note that the reduction from \fvs to \submodcover which follows from this connection does not seem to be well-known in the literature, and the authors of 
this paper were not aware of it until recently.
\end{remark}


From a structural point of view we
also prove that \submodcover reduces to \rhosdds{1}, thus essentially showing the
equivalence of \submodcover and \sdds. We believe that it is useful to have this equivalence explicitly known given that vertex deletion problems arise naturally but seem different from covering problems on first glance.

\begin{restatable}{theorem}{thmSubmodCovertosdds}\label{thm:SubmodCovertosdds}
Let $h: 2^V\rightarrow \Z_{\ge 0}$ be an integer-valued normalized non-decreasing submodular function. Then, there exists a normalized supermodular function $f:2^V\rightarrow \Z_{\ge 0}$ 
% \knote{$f:2^V\rightarrow \Z_{\ge 0}$} \knote{edit proof accordingly} 
such that 
\begin{enumerate}
    \item for $F\subseteq V$, we have that $h(F)\ge h(V)$ if and only if $\lambda^*_{f|_{V-F}}\le 1$, 
    \item %$\max\{f(v|V-v): v\in V\}\le \max\{h(v): v\in V\}+1$.
    $f(v|V-v) = h(v) + 1$ for all $v \in V$, and 
    \item evaluation queries for the function $f$ can be answered in polynomial time by making a   constant number of evaluation queries to the function $h$. 
\end{enumerate}
\end{restatable}

\subsubsection{Approximation Hardness}
A starting point for our attempt to answer Question~\ref{question:main} was
our belief that $\rho$-\dds for integer $\rho$ admits a $(\rho+1)$-approximation
via the primal-dual approach suggested by Fujito for \mfvs \cite{Fujito-matroid-fvs}. This belief stems from Fujito's work which showed a $2$-approximation for vertex cover, \fvs, \pfds, and \mfvs for  ``uniformly sparse'' matroids and our reduction showing that $\rho$-\dds for integral $\rho$ is a special case of \mfvs (see Theorem \ref{thm:dds-to-matroidfvs}). We note that the matroid that arises in the reduction is not a ``uniformly sparse'' matroid but has lot of similarities with it, so we our initial belief was that a more careful analysis would lead to a constant factor approximation. 
However, to our surprise, after several unsuccessful attempts to prove a constant factor
upper bound, we were able to show that for every integer $\rho \geq 2$,  $\rho$-\dds is $\Omega(\log n)$-hard to approximate via a reduction from Set Cover. 

\begin{restatable}{theorem}{thmDDSlognHard}\label{thm:DDS-logn-hard}
For every integer $\rho \geq 2$,  there is no $o(\log n)$ approximation for \rhodds{\rho} assuming $P\neq NP$, where $n$ is the number of vertices in the input instance.
\end{restatable}

Thus, $\rho$-\dds exhibits a \emph{phase transition}: it admits a $2$-approximation for $\rho\le 1$ (via Fujito's results \cite{Fujito-matroid-fvs}) and becomes $\Omega(\log{n})$-hard for every integer $\rho\ge 2$. To conclude our hardness results, we note that since \dds is a special case of  \mfvs, which itself is a special case of \sdds, both \mfvs and \sdds are $\Omega(\log n)$-inapproximable. However, both these problems are also $O(\log{n})$-approximable via Corollary \ref{coro:rhodds-and-mfvs}. Thus, we resolve the approximability of all these problems to within a small constant factor. We refer the reader to Figure \ref{fig:reductions} for an illustration of problems considered in this work and approximation-factor preserving reductions between them.
% \knote{I edited this paragraph.}

\iffalse
\knote{Move the conjecture to conclusion section and mention the result for $\rho\ge 3$ there. Better to focus on $\rho$ being an integer here. This is the case related to matroids too.}
In fact, we were able to strengthen our reduction of \Cref{thm:DDS-logn-hard} to additionally show that  for every rational \emph{constant} $\rho \geq 3$,  $\rho$-\dds is $\Omega(\log n)$-hard to approximate.  Due to this and other related technical considerations, we raise the following conjecture.
\begin{conjecture}\label{conj:phase-transition}
For every rational constant $\rho > 1$,  there is no $o(\log n)$ approximation for \rhodds{\rho} assuming $P\neq NP$, where $n$ is the number of vertices in the input instance.
\end{conjecture}

Proving \Cref{conj:phase-transition} would result in the following interesting \emph{phase-transition} phenomenon: $\rho$-\dds admits a $2$-approximation for $\rho\le 1$ (via Fujito's results \cite{Fujito-matroid-fvs}) and becomes $\Omega(\log{n})$-hard for \emph{every} $\rho>1$.  Since our proof of the generalization of \Cref{thm:DDS-logn-hard} is technically involved and we were unable to fully extend it for the entire parameter range of \Cref{conj:phase-transition}, in this version we restriction attention to the hardness for integer values of $\rho$. 
% \knote{Omit which result/proof? Confusing.} \cnote{Yes, confusing. How about the followoing: In this version we restriction attention to the hardness for integer values of $\rho$.}

To conclude our hardness results, we note that since \dds is a special case of  \mfvs, which itself is a special case of \sdds,
 both \mfvs and \sdds are $\Omega(\log n)$-inapproximable. However, both these problems are also $O(\log{n})$-approximable via 
Corollary \ref{coro:rhodds-and-mfvs}. 
Thus, we resolve the approximability of all these problems to within a small constant factor. 
We refer the reader to Figure \ref{fig:reductions} for an illustration of problems considered in this work and approximation-factor preserving reductions between them. 
\fi

\begin{figure}[ht]
\centering
\includegraphics[width=0.8\textwidth, trim={2cm 1cm 4cm 2.5cm}, clip]{Full-version/technical-sections/diagrams/dds-diagram-connections.pdf}
\caption{Reductions between problems of interest to this work. Arrow from Problem A to Problem B implies that Problem A has an approximation-preserving reduction to Problem B. Figure (a) consists of the connections between problems known prior to our work. Figure (b) showcases our results.}
%The reductions from \dds to \mfvs and from \mfvs to \sdds indicated by thick lines are non-trivial observations can be found in \Cref{appendix:sec:reductions}.}
\label{fig:reductions}
\end{figure}
% \knote{Edit caption to cite appendix.}

\subsubsection{Bicriteria Approximations}
The hardness result for $2$-\dds (and $\rho$-\dds) motivates us to consider bicriteria approximation algorithms. Can we obtain constant factor approximation by relaxing the requirement of meeting the density target $\rho$ exactly? We show that this is indeed possible.
We consider an orientation based  LP that was used recently to obtain a polynomial-time solvable LP to approximate \fvs and \pfds \cite{chandrasekaran2024polyhedralaspectsfeedbackvertex}.
We observed that this LP has an $\Omega(n)$ integrality gap when considering $2$-\dds. Nevertheless, the LP is useful in obtaining the following bicriteria approximation.

\begin{restatable}{theorem}{thmbicriteriaorientation}\label{thm:orientation-LP-bicriteria}
    There exists a polynomial time algorithm which takes as input a graph $G = (V, E)$, vertex deletion costs $c:V\rightarrow\R_{\ge 0}$, a target density $\rho\in \R$, and an error parameter $\epsilon \in (0, 1/2)$, and returns a set $S\subseteq V$ such that:
    \begin{enumerate}
        \item $\lambda^*_{G - S} \leq \left(\frac{1}{1 - 2\epsilon}\right) \cdot \rho$,
        \item $\sum_{u\in S}c_u \leq \left(\frac{1}{\epsilon}\right) \cdot \mathtt{OPT}$,
    \end{enumerate}
    where \texttt{OPT} denotes the cost of an optimum solution to \rhodensitydeletionset on the instance $(G,c)$.
\end{restatable}


Next, we consider $\rho$-\sdds. Unlike the case of graphs, it is not clear how to write an integer programming formulation for \sdds whose LP-relaxation is polynomial-time solvable. Instead, 
we take inspiration from the very recent work of \cite{Włodarczyk_2024} on vertex deletion to reduce treewidth. We design a
combinatorial randomized algorithm that yields a bicriteria approximation for \sdds, where the bicriteria approximation bounds are based on a parameter $c_f$ that depends on the input supermodular function $f$. 
For a normalized supermodular function $f:2^V\rightarrow\R_{\ge 0}$, we define 
        \[c_f := \max\left\{\frac{\sum_{u \in S}f(u|S-u)}{f(S)}: S\subseteq V\right\}.
        \]
This parameter $c_f$ was defined in a recent work 
on \dss to unify the analysis of the greedy peeling algorithm for \dsg \cite{cqt-22}. 
We note that $1 \leq c_f \leq |V|$ and moreover, $c_f = 1$ if and only if the function $f$ is modular. If $f$ is the induced edge function of a graph (i.e., $f(S)$ is the number of edges with all its end-vertices in $S$ for every subset $S$ of vertices), then $c_f \le 2$. This follows from the observation that the sum of degrees is at most twice the number of edges in a graph. Similarly, if $f$ is the induced edge function of a hypergraph with rank $r$ (i.e., all hyperedges have size at most $r$), then $c_f \leq r$. 
We show the following bicriteria approximation for \sdds. 

\begin{restatable}{theorem}{thmbicriteriarandomdeletion}\label{thm:bicriteria-random-deletion}
    There exists a randomized polynomial time algorithm which takes as input a normalized  monotone supermodular function $f:2^V\rightarrow\Z$ (given by oracle access), element deletion costs $c:V\rightarrow\R_{\ge 0}$, a target density $\rho\in \R$, and an error parameter $\epsilon \in (0, 1)$, and returns a set $S\subseteq V$ such that:
    \begin{enumerate}
        \item $\lambda^*_{f|_{V - S}} \leq c_f(1+\epsilon)\cdot \rho$,  and 
        \item $\E\left[\sum_{u\in S}c_u\right] \leq c_f \left(1+\frac{1}{\epsilon}\right)\cdot \mathtt{OPT}$,
    \end{enumerate}
    where \texttt{OPT} denotes the cost of an optimum solution to \rhosdds{\rho} on the instance $(f,c)$.
\end{restatable}

As a consequence of Theorem \ref{thm:bicriteria-random-deletion}, we obtain a bicriteria approximation for density deletion problems in graphs and $r$-rank hypergraphs. We note that the bicriteria guarantee that we get from this theorem for graphs is weaker than the guarantee stated in Theorem \ref{thm:orientation-LP-bicriteria}. 
We discuss another special case of \sdds where the supermodular function of interest has bounded $c_f$ to illustrate the significance of Theorem \ref{thm:bicriteria-random-deletion}. Given a graph $G=(V, E)$ and a parameter $p\ge 1$, the $p$-mean density of $G$ is defined as $\max\{\sum_{u\in S}d_S(u)^p/|S|: S\subseteq V\}$, where $d_S(u)$ is the number of edges in $E[S]$ incident to the vertex $u$. The $p$-mean density of graphs was introduced and studied by Veldt, Benson, and Kleinberg \cite{vbk-21}. Subsequent work by Chekuri, Quanrud, and Torres \cite{cqt-22} showed that $p$-mean density is a special case of the densest supermodular set problem (i.e., \dss) where the supermodular function $f: 2^V\rightarrow \R_{\ge 0}$ of interest is given by $f(S):=\sum_{u\in S}d_S(u)^p$ for every $S\subseteq V$ and moreover $c_f\le (p+1)^p$. We note that the natural vertex deletion problem is the $p$-mean density deletion problem: 
given a graph $G=(V, E)$ with vertex deletion costs, 
find a min-cost subset of vertices to delete so that the $p$-mean density of the remaining graph is at most a given threshold. Since $c_f\le (p+1)^p$ for the function $f$ of interest here, Theorem \ref{thm:bicriteria-random-deletion} implies a bicriteria approximation for $p$-mean density deletion  for integer-valued $p$. 
An interesting open question is to obtain better bicriteria approximation for \rhosdds{\rho}---in particular, can we remove the dependence on $c_f$? %\knote{State this open question in the conclusion as well.}

\subsection{Preliminaries: Characterizing Density Using Orientations}
In this section, we give a characterization of density via \emph{(fractional) orientations} which we use throughout the technical sections. We recall that an \emph{orientation} of a graph $G=(V,E)$
assigns each edge $\{u,v\}$ to either $u$ or $v$. A \emph{fractional orientation} is an assignment of
two non-negative numbers $z_{e,u}$ and $z_{e,v}$ for each edge $e=\{u,v\} \in E$ such that 
$z_{e, u}+ z_{e,v}=1$. We note that an orientation is a fractional orientation where all values in the assignment are either $0$ or $1$. For notational convenience, we use $\vec{G} = (V, \vec{E})$ to denote an orientation of the graph $G$ and $\indegree_{\vec{G}}(u)$ to denote the indegree of a vertex $u \in V$ in the oriented graph $\vec{G}$.
% The following characterization implied by the dual of Charikar's \cite{charikar_greedy_2000}  LP to solve \dsg.
% \begin{proposition}\label{thm:Charikar-fraction-orientation}
% Let $G=(V, E)$ be a graph. We have that $\lambda^*_G\le \rho$ if and only if there exists a fractional orientation $z$ such that
% $\sum_{e\in \delta(u)}z_{e,u}\le \rho$ for every $u\in V$. 
% \end{proposition}
The following connection between density and (fractional) orientations will be used in our hardness reduction in \Cref{sec:set-cover-hardness}, our ILP in  \Cref{sec:orientation-bicriteria}, and the connection between \rhodensitydeletionset and \mfvs in \Cref{appendix:sec:reductions}.
\begin{proposition}\label{thm:orientation-characterization}
Let $G=(V, E)$ be a graph. Then, we have the following:
\begin{enumerate}
    \item let $\rho \in \R_{\geq 0}$ be a real value; then, $\lambda^*_G\le \rho$ if and only if there exists a fractional orientation $z$ such that $\sum_{e\in \delta(u)}z_{e,u}\le \rho$ for every $u\in V$, and
    \item let $\rho \in \Z_{\geq 0}$ be an integer value; then, $\lambda^*_G\le \rho$ if and only if there exists an orientation $\vec{G} = (V, \vec{E})$ of the graph $G$ such that $\indegree_{\vec{G}}(u) \leq \rho$ for every $u\in V$.
\end{enumerate}
\end{proposition}
The first part of the proposition states that a graph $G$ has density at most $\rho$
if and only if the edges of $G$ can be fractionally oriented such that the total fractional in-degree at every vertex is at most $\rho$. This characterization is implied by the dual of Charikar's LP \cite{charikar_greedy_2000} to solve \dsg.
The second part of the proposition is a strengthening of the first part when $\rho$ is an integer and states that a graph $G$ has density at most $\rho$ iff the edges of $G$ can be (integrally) oriented such that the in-degree at every vertex is at most $\rho$.  This characterization is implied by a result of Hakimi \cite{Frank-book} and also via the dual of Charikar's LP \cite{charikar_greedy_2000}.  
% Then, the third part of the proposition, along with the second part, implies that a graph is a pseudoforest iff its edges can be oriented such that the maximum indegree is at most $1$ (see \cite{chandrasekaran2024polyhedralaspectsfeedbackvertex} for additional details).

==> preliminaries.tex <==

%\subsection{Preliminaries}\label{sec:prelim}

%\paragraph{Organization.}

%\cnote{I removed the subsection title and edited the para/theorem below.}
\paragraph{Fractional orientations.}
We rely on a characterization of $\lambda^*_G$ via fractional orientations. This is
implied via the dual of Charikar's \cite{charikar_greedy_2000} 
LP to solve \dsg. Recall that an orientation of a graph $G=(V,E)$
assigns each edge $\{u,v\}$ to either $u$ or $v$. A fractional orientation is an assignment of
two non-negative numbers $z_{e,u}$ and $z_{e,v}$ for each edge $\{u,v\} \in E$ such that 
$z_{e, u}+ z_{e,v}=1$.

\begin{theorem}\label{thm:Charikar-fraction-orientation}
Let $G=(V, E)$ be a graph. We have that $\lambda^*_G\le \rho$ if and only if there exists a fractional orientation $z$ such that
$\sum_{e\in \delta(u)}z_{e,u}\le \rho$ for every $u\in V$. 
\end{theorem}
The theorem states that a graph $G$ has density at most $\rho$
if and only if the edges of $G$ can be fractionally oriented such that the total fractional in-degree at every vertex is at most $\rho$.   


\iffalse
\begin{theorem}\label{thm:Charikar-fraction-orientation}
Let $G=(V, E)$ be a graph. We have that $\lambda^*_G\le \rho$ if and only if there exists $z_{e,u}\in [0, 1]$ for every $u\in e\in E$ such that $z_{e, u}+ z_{e,v}=1$ for every $e=\{u,v\}\in E$ and $\sum_{e\in \delta(u)}z_{e,u}\le \rho$ for every $u\in V$. 
\end{theorem}


This interpretation leads to Theorem \ref{thm:Charikar-fraction-orientation} below which we will leverage heavily throughout the technical sections. Equivalently, the theorem states that a graph $G$ has density at most $\rho$
if and only if the edges of $G$ can be fractionally oriented such that the total fractional in-degree at every vertex is at most $\rho$.   
\fi


%\paragraph{Problem Definitions.} For our inapproximability results, we will need the following problem definition.



%\knote{The only preliminary that is used across multiple sections is the orientatoin LP. Keep that here. Move rest of the preliminaries to relevant sections.}




==> reductions-diagram.tex <==
\begin{figure}[h!]\label{fig:problem-relationships}
\centering
\begin{tikzpicture}[
  every node/.style={draw, rectangle, rounded corners, align=center},
  ->
]

% Nodes
\node (vc) {Vertex Cover};
\node (sc) [below left=of vc] {Set Cover};
\node (fvs) [below right=of vc] {Feedback Vertex Set};
\node (pds) [below=of fvs] {Pseudoforest Deletion Set};
\node (dds) [below=of sc] {Density Deletion Set};
\node (mfvs) [below left=of dds] {Matroid Feedback Vertex Set};
\node (smds) [below right=of dds] {Supermodular Density Deletion Set};
% \node (smvs) [below=of smds] {Supermodular Deletion Set};
\node (scov) [below right=of mfvs] {Submodular Cover};

% Arrows showing relationships
\draw[->] (vc) -- (sc);
\draw[->] (vc) -- (fvs);
\draw[->] (fvs) -- (pds);
\draw[->] (sc) -- (dds);
\draw[->] (pds) -- (dds);
\draw[->] (dds) -- (mfvs);
% \draw[->] (dds) -- (smvs);
\draw[->] (dds) -- (smds);
\draw[->] (mfvs) -- (scov);
% \draw[->] (smvs) -- (scov);
\draw[->] (smds) -- (scov);

\end{tikzpicture}
\caption{Relationships amongst problems. 
%We note that all problems are NP-hard and so polynomially equivalent to each other in the exact sense. 
An arrow from Problem A to Problem B indicates that Problem A can be reduced to Problem B in an approximation-preserving manner.}
\end{figure}

==> technical-sections/dense-subgraph-decomposition.tex <==
\subsubsection{Dense Decompositions}



In this section, we show that we can preprocess the input graph $G = (V, E)$ so that it satisfies certain useful properties. In particular, we show the following:

\begin{lemma}\label{lem:preprocess-dsd}
    Let $G = (V, E)$ be a graph and $\rho \in \Z_+$ be a positive integer such that $\density(G) > \rho$. Then, there exists $R \subseteq V$ such that:
    \begin{enumerate}
        \item Every solution for \rhodensitydeletionset in $G[R]$ is a solution for \rhodensitydeletionset in $G$, and
        % \item There exists a fractional orientation of $\vec{E}[R]$ such that $\indegree_{\vec{E}[R]}(u) > \rho$ for all $u \in R$,
        % \item There exists an integral orientation of $\vec{E}[R]$ such that $\indegree_{\vec{E}[R]}(u) \geq \rho$ for all $u \in R$, and
        \item $\rank_{\calM|_{G[R]}}(E[R]) = \rho|R|$.
    \end{enumerate}
    Moreover, such a set $R$ can be found in polynomial time.
\end{lemma}

